Speculative Coreset Selection for Task-Specific Fine-tuning

Task-specific fine-tuning is essential for the deployment of large language models (LLMs), but it requires significant computational resources and time. Existing solutions have proposed coreset selection methods to improve data efficiency and reduce model training overhead, but they still have limitations: 1) Overlooking valuable samples at high pruning rates, which degrades the coreset's performance. 2) Requiring high time overhead during coreset selection to fine-tune and evaluate the target LLM. In this paper, we introduce STAFF, a speculative coreset selection method. STAFF leverages a small model from the same family as the target LLM to efficiently estimate data scores and then verifies the scores on the target LLM to accurately identify and allocate more selection budget to important regions while maintaining coverage of easy regions. We evaluate STAFF on three LLMs and three downstream tasks and show that STAFF improves the performance of SOTA methods by up to 54.3% and reduces selection overhead by up to 70.5% at different pruning rates. Furthermore, we observe that the coreset selected by STAFF at low pruning rates (i.e., 20%) can even obtain better fine-tuning performance than the full dataset.

==> src/related.tex <==
\section{Related work}
\label{sec:related}

{\bf Coreset Selection.}
Coreset selection has been widely used in machine learning and deep learning~\citep{chai2023efficient,sener2018active,xia2022moderate}.
In addition to the aforementioned work, researchers have proposed various methods to select important, difficult, or diverse data to improve data efficiency~\citep{xia2022moderate,coleman2019selection,pleiss2020identifying}.
However, these methods are usually designed for classification tasks and are susceptible to catastrophic performance degradation at high pruning rates.
In addition, existing work also utilizes optimization techniques to optimize the data coreset, thereby minimizing empirical risks~\citep{DBLP:conf/nips/PruthiLKS20,yang2023dataset,killamsetty2021grad}.
However, such complex optimization methods require cumbersome calculations and can hardly be applied to task-specific LLM fine-tuning.
In this paper, we utilize small models to select the coreset taking account of both data diversity and importance, and achieve better-performing data selection with lower overhead than state-of-the-art methods.

{\bf LLM Data Pruning.}
Researchers have designed various data selection and pruning methods to improve the data quality and efficiency for LLM training, covering different settings like pre-training~\citep{xie2023data,marion2023less,xie2023data,DBLP:conf/nips/PenedoMHCACPAL23}, instructional fine-tuning~\citep{liu2023makes,muennighoff2023octopack,lu2023instag,wang2022self,yang2024smalltolarge}, and preference fine-tuning~\citep{ethayarajh2024kto,pace2024west,kim2023prometheus,cui2023ultrafeedback}.
This paper focuses on coreset selection for task-specific fine-tuning on various downstream tasks.
% \citet{yang2024smalltolarge} use the training trajectories from
% small models to guide data clustering and selection for the LLM on the MathInstruct dataset.
\citet{lin2024data} have proposed a data selection method for the recommendation task of LLM systems based on the influence score and effort score. However, their method can hardly adapt to other tasks.



{\bf Speculative Execution in LLM.}
The concept of \textit{speculative execution} has been widely used in LLM to improve the quality and efficiency of decoding and reasoning.~\citep{miao2024specinfer,leviathan2023fast,hooper2023speed,li2024purifying,DBLP:conf/acl/XiaYDW00L0S24,DBLP:conf/acl/Zhang00S0CM24,li2024specpim}.
\citet{miao2024specinfer} propose SpecInfer that first uses the small speculative models to generate the token tree and then proposes multi-step speculative sampling and parallel decoding to efficiently verify the token tree.
Inspired by the concept of \textit{speculative execution}, in this paper, we use small models to calculate data score and perform verification and coreset selection on the target LLM, thereby achieving better results than existing methods while significantly reducing the selection overhead.


% \section{Discussion}
% \label{sec:discuss}

% {\bf Using on small models.} This paper introduces \sys that utilizes a smaller model in the same family as the target LLM to select the coreset for task-specific fine-tuning of the target LLM.
% However, \sys cannot be directly applied to LLMs without any smaller model in the family.
% Using model pruning to build small models or selecting models from other families are potential solutions.
% Studying the impact of pruned models and models in another family on coreset selection and improving the selection method will be a future research direction.

% {\bf Impact of small model capability.}
% The capability of the small model significantly impacts the effectiveness of \sys.
% A less capable small model cannot effectively learn knowledge from downstream tasks, thus failing to provide meaningful scores to guide data selection for the target LLM, leading to results close to the random selection, as shown in the last row of~\autoref{tab:rq2}.
% % How to evaluate and select small models before experiments will be a valuable improvement in the future. Additionally, 
% \citet{miao2024specinfer} proposes to combine multiple small models to achieve better performance in LLM speculative decoding, providing a potential direction for improving \sys.

% {\bf Using on small models.}
% % 1. this method is not available for finetuning the small models, which can not find another small one as speculative model

% {\bf Impact of small model capability.}
% % 2. the finetuning results of the small model have a significant impact on the effectiveness of \sys

==> tftex/rq1-1.tex <==
\begin{table}[]
    \caption{Performance comparison between \sys and best baseline CCS under 90\% pruning rate on the Gemma-7b model. The symbols \(\uparrow\) and \(\downarrow\) separately indicate whether a higher or lower value of a specific metric is preferable. `\% Improve' denotes the relative improvement achieved by \sys compared with the best baseline method. \looseness=-1}
    \scriptsize
    \label{tab:rq1-1}
    \centering
    \tabcolsep=2pt
\begin{tabular}{cccccccccc}
\toprule
\multirow{2}{*}{} & \multicolumn{3}{c}{\textbf{BioInstruct}} & \multicolumn{3}{c}{\textbf{DialogSum}} & \multicolumn{3}{c}{\textbf{WMT}} \\ \cmidrule(r){2-4} \cmidrule(r){5-7} \cmidrule(r){8-10}
 & \textbf{Rouge-L \(\uparrow\)} & \textbf{BLEU-4 \(\uparrow\)} & \textbf{SEL. Time (h) \(\downarrow\)} & \textbf{Rouge-L \(\uparrow\)} & \textbf{BLEU-4 \(\uparrow\)} & \textbf{SEL. Time (h) \(\downarrow\)} & \textbf{Rouge-L \(\uparrow\)} & \textbf{BLEU-4 \(\uparrow\)} & \textbf{SEL. Time (h) \(\downarrow\)} \\  \midrule
% Full & 41.8 & 47.4 & - & 49.8 & 52.8 &  & 62.2 & 68.8 & - \\
\textbf{CCS} & 39.3 & 45.2 & 5.4 & 47.4 & 50.3 & 4.8 & 54.1 & 61.4 & 8.9 \\
\textbf{\sys} & 39.4 & 46.2 & 3.1 & 48.4 & 51.1 & 3.0 & 55.9 & 63.3 & 3.5 \\ \midrule
\textbf{Impr. (\%)} & 0.2 & 2.2 & 42.6 & 2.2 & 1.5 & 36.4 & 3.3 & 3.1 & 61.0 \\ \bottomrule
\end{tabular}
% \vspace{-0.1cm}
\end{table}

